Reinforcement Learning for Low-Thrust Trajectory Design of Interplanetary Missions

This paper investigates the use of Reinforcement Learning for the robust design of low-thrust interplanetary trajectories in presence of severe disturbances, modeled alternatively as Gaussian additive process noise, observation noise, control actuation errors on thrust magnitude and direction, and possibly multiple missed thrust events. The optimal control problem is recast as a time-discrete Markov Decision Process to comply with the standard formulation of reinforcement learning. An open-source implementation of the state-of-the-art algorithm Proximal Policy Optimization is adopted to carry out the training process of a deep neural network, used to map the spacecraft (observed) states to the optimal control policy. The resulting Guidance and Control Network provides both a robust nominal trajectory and the associated closed-loop guidance law. Numerical results are presented for a typical Earth-Mars mission. First, in order to validate the proposed approach, the solution found in a (deterministic) unperturbed scenario is compared with the optimal one provided by an indirect technique. Then, the robustness and optimality of the obtained closed-loop guidance laws is assessed by means of Monte Carlo campaigns performed in the considered uncertain scenarios. These preliminary results open up new horizons for the use of reinforcement learning in the robust design of interplanetary missions.

==> PPO.tex <==


Policy-based RL

In an episodic environment, a natural measurement is the start value of the policy, which is the expected value of the start state:

$$J_1(\theta) = V_{\pi_\theta}(s_1) = E \pi \theta [v_1] $$


$$ E_{\tau \sim \pi_\theta} $$


PPO employs a clipped surrogate objective to prevent the new policy from straying away from the old one. The clipped objective function of state-action ($s_t$, $a_t$) is

Weighted combination of n-step returns
\begin{align}
   A_{GAE} = \sum_n {w_n \hat A_n^\pi (s_t, a_t)} \\
   w_n = \lambda^{n-1} \\
   %
   \hat A_{GAE} \sum_{t'=t}^N (\gamma \lambda)^{t'-t} \delta_{t'} \\
    \delta_{t'} = r(s_{t'}, a_{t'}) + \gamma \hat V_\phi^\pi(s_{t'+1}) - \hat V_\phi^\pi(s_{t'}) 
\end{align}

 



Policy gradient methods work by computing an estimator of the policy gradient and plugging it
into a stochastic gradient ascent algorithm. The most commonly used gradient estimator has the
form








A state-of-the-art policy gradient method named Proximal Policy Optimization~\cite{schulman2017proximal} is adopted in this paper because of the high performance demonstrated on a number of continuous and high-dimensional control problems.







Policy gradient methods works by running the current policy $\pi_{\theta_j}$ in $n_{env}$ independent realizations of the environment for $n_b$ training episodes \hl{each/each one}, and collecting a set of trajectories $\{ \tau_i\}_{i = 1, \dots, n_{env} n_b}$. At the end of the sampling process, the policy performance are evaluated by using a policy performance index that has typically the form:
\hl{controllare bene, non mi torna}
\begin{equation}
    J(\theta_j) =  \underset{\tau \sim \pi_{\theta_j}}{\mathbb{E}}\left[\sum_{k = 0}^{N} \log{\pi_{\theta_j}(\bm{a}_k | \bm{s}_k)} \hat{A}_{k}\right]
    \label{eq:Jvan}
\end{equation}
where $\tau = (\bm{s}_0, \bm{a}_0, \bm{s}_1, \bm{a}_1, \dots)$ represents a trajectory, $\pi_\theta(\bm{a}_k | \bm{s}_k)$ is a stochastic policy, that express the probability of taking action $\bm{a}_k$ in state $\bm{s}_k$, and $\hat{A}_k$ is an estimator of the advantage function, defined as:
\begin{equation}
    A^\pi(\bm{s}_k, \bm{a}_k) = Q^\pi(\bm{s}_k, \bm{a}_k) - V^\pi(\bm{s}_k)
\end{equation}
which expresses by how much the total reward improves by taking a specific action $\bm{a}_k$ in state $\bm{s}_k$ instead of randomly selecting the action according to $\pi_\theta(\cdot|\bm{s}_k)$.
From a computational point of view, the advantage function is usually approximated by using the so-called generalized advantage estimation:
\begin{align}
    \hat{A}_k &= \sum_{k'= k}^{N-1} (\gamma \lambda)^{k'-k} \delta_{k'} \\
    \delta_k &= r_k + \gamma V_\phi(\bm{s}_{k+1}) - V_\phi(\bm{s}_{k})
\end{align}

\hl{questa non la so, va controllata}
%\hl{delta dovrebbe essere qualcosa come temporal difference TD($\lambda$). Si dimostra che E[delta] = A.}

At this point, the policy parameters $\theta$ are updated via stochastic gradient ascent on that performance index:
\begin{equation}
    \theta_{j+1} = \theta_{j} + \alpha \nabla_\theta J(\theta)|_{\theta_j}
\end{equation}
where $\alpha$ indicates the learning rate, that usually is a decreasing function of the training step number.
In an analogous way, the value function parameters $\phi$ are updated via gradient descent on the mean-squared error $E(\phi)$ between the current estimate of value function and the rewards-to-go, that is:
\begin{equation}
    E(\phi) = \underset{\tau \sim \pi_{\theta}}{\mathbb{E}}\left[ \frac{1}{N} \sum_{k = 0}^{N} \left(V_\phi (\bm{s}_k) - \sum_{k' = k}^{N} r_{k'} \right)^2 \right]
\end{equation}

The problem with performance index \eqref{eq:Jvan} is that, empirically, it tends to perform too large policy updates, which are often the cause of performance collapse.
PPO was created with the aim of improving the stability of policy-gradient methods by avoid having too large policy updates. 
This is accomplished by using a so-called ``clipped surrogate objective function'' $J^{clip}$ in place of $J$, that constraints the updated policy $\pi_{\theta_j}$ to stay in a small range $\epsilon$, named clip range, around the previous value $\pi_{\theta_{j-1}}$, by clipping the probability that the new policy moves outside of interval $[1-\epsilon, 1+\epsilon]$.
So, by introducing a probability ratio
\hl{gli serve un simbolo migliore perche' $r$ lo abbiamo usato per il raggio}:
\begin{equation}
    r_k(\theta_j) = \frac{\pi_{\theta_j}(\bm{a}_k | \bm{s}_k)}{\pi_{\theta_{j-1}}(\bm{a}_k | \bm{s}_k)}
\end{equation}
the clipped objective function can be written as:
\begin{equation}
    J^{clip}(\theta_j) =  \underset{\tau \sim \pi_{\theta_j}}{\mathbb{E}}\left[ \frac{1}{N} \sum_{k = 0}^{N}  \min{\left( r_k(\theta_j) \hat{A}_k, \mbox{clip}(r_k(\theta_j), 1-\epsilon, 1+\epsilon) \hat{A}_k\right)} \right]
\end{equation}
In the same fashion as the learning rate, also the clip range $\epsilon$ can be a decreasing function of the training step number.
Typically, in PPO the policy and value-function update is done all at once by gathering in the set of parameters $\theta$ the weights and biases of both the actor and critic networks, and including the value function error term $E$ in the objective function. Eventually, an entropy term $S$ is added to ensure sufficient exploration, bringing to the final surrogate objective function:
\begin{equation}
    J^{ppo}(\theta_j) = J^{clip}(\theta_j) - c_1 E(\theta_j) + c_2 S(\theta_j)
\end{equation}
where $c_1$ and $c_2$ are two hyperparameters named value function coefficient and entropy coefficient, respectively.
Moreover, with respect to classical policy gradient methods, in PPO the policy update is performed by running $n_{opt}$ epochs of stochastic gradient descent over $n_b$ sampling mini-batches, each with $n_{env}N$ training samples.
The algorithm terminates after a total number of training steps equal to $M$.

As a final remark, it is worth noting that the RL algorithm just presented is completely model-free, as it does not depend in any way on the mathematical form of the transition function $f$, control model $g$ and observation model $h$, nor on the expression of the probability distributions $P$.



\section{SCARTI}



\subsection{\hl{--------------------}}

 


 







Reducing Variance Using a Baseline

We subtract a baseline function B(s) from the policy gradient
This can reduce variance, without changing expectation


A good baseline is the state value function $B(s) = V^{\pi_\theta}(s)$

So we can rewrite the policy gradient using the advantage
function 
$$A^{\pi_\theta} = Q^{\pi_\theta}(s, a) - V^{\pi_\theta}(s)$$


For the true value function $V^{\pi_\theta}(s)$, the TD error $\delta^{\pi_\theta}$ is

$$\delta^{\pi_\theta} = r + \gamma V^{\pi_\theta}(s') - V^{\pi_\theta}(s)$$

is an unbiased estimate of the advantage function, that is $E_{\pi_\theta}[\delta^{\pi_\theta}] = A^{\pi_\theta}(s,a)$.

In practice we can use an approximate TD error
$$
\hat \delta = r + \gamma  V_\phi(s') - V_\phi(s)
$$
and then use the (approximated) TD error to compute the policy gradient
 $$
 \nabla_\theta J(\theta) = E \left[ \nabla_\theta log {\pi_\theta}(s,a) \hat \delta\right]
 $$

This approach only requires one set of critic parameters $\phi$






 


%While Monte Carlo methods only adjust their estimates once the final outcome is known, TD methods adjust predictions to match later, more accurate, predictions about the
% TD method bases its update in part on an existing estimate,
%we say that it is a bootstrapping method
%$$ g =\mathbb{E} \left[\nabla_\theta \log \pi_\theta(s, a)  \mathbb{E} \sum_{t' = t}^N r_{t'}-b(s_t) \right] $$
%
%Combining these two improvement one has $g =\mathbb{E} \left[\nabla_\theta \log \pi_\theta(s, a)  \hat A(s_t, a_t) \right] $











proximal policy optimization (PPO) simplifies Trust region policy optimization (TRPO) (Schulman, et al., 2015) 
 using a clipped surrogate objective while retaining similar performance.








The goal is thus to chose $\theta$ 

The value of the reward (objective) function depends on this policy and then various algorithms can be applied to optimize $\theta$ for the best reward.



In high-dimensional spaces or complex environments,






the agent  attempt at  learning the control policy $\pi(\bm{s})$ .
instead of learning the (e.g., Deep Q Network, DQN)




model-free RL approaches dos not rely on an \textit{a-priori} knowledge of the transition function $f$, control model $g$, and observation model $h$, nor of the probability distributions of disturbance $P$ (see Eq.s~\eqref{eq:MDP}-\eqref{eq:MDP2}) and work even in case these function are non-analytical.
\hl{questo e' utile per questo problema perche'}




 

 \hl{-------------------------------------}
 















 \hl{-------------------------------------}
The environment initializes an episode by randomly generating an internal state, mapping this
internal state to an observation, and passing the observation to the agent.

 At each step of the episode, an observation is generated from
the internal state and given to the agent. The agent uses this observation to generate
an action that is sent to the environment; the environment then uses the action and the
current state to generate the next state and a scalar reward signal. The reward and the
observation corresponding to the next state are then passed to the agent



 
 
  The DNNs can be Feedforward Networks (FNNs), as Multi-Layer Perceptron (MLP) networks, as well as recurrent networks, as Long-Short Term Memory (LSTM) networks. 
  
  
 
 n this context, the term \gncnet{} (namely, Guidance and Control Network) was coined at the European Space Agency \cite{izzo2019survey} to refer to a Deep Neural Network (DNN) used to map any observation $\bm{o}_k$ of the spacecraft state $\bm{s}_k$ (e.g., position, velocity and mass) to the corresponding (parameterized) policy $\pi_\theta(\bm{s}_k)$ (e.g., the thrust vector) and/or (parameterized) value function $V_\phi(\bm{s}_k)$.
%, that is, the overall performance score that is expected by following the optimal policy starting from that state
 
 The computational effort is mainly spent on the network training, which has to be performed just once. After training, the \gncnet{} can be used to evaluate an optimal state-feedback control policy at almost no computational cost. This feature makes the \gncnet{} also suitable to be used as an integrated on-board guidance and control system during the cruise phase of interplanetary missions, providing the spacecraft with the capability of autonomously adjusting its trajectory in situations where corrective commands from Earth are not possible, such as during a short-duration maneuver (e.g., the flyby of an asteroid) or when the number of available radio links with Earth is limited. Furthermore, the trained network is able to run also on cheaper processors, as those typically mounted on-board of micro-spacecraft because of the limited budget.
 
 
 
 

 
 
 
 
 \hl{---------------------------------}
 



In order to avoid having a third DNN,
the 

One may easily prove that

the TD error $\delta^{\pi_\theta} = r + \gamma V^{\pi_\theta}(s') - V^{\pi_\theta}(s)$ is
is an unbiased estimate of the advantage function, that is $E_{\pi_\theta}[\delta^{\pi_\theta}] = A^{\pi_\theta}(s,a)$.
Hence,



For the true value function $V^{\pi_\theta}(s)$, the TD error $\delta^{\pi_\theta}$ is


In practice we can use an approximate TD error
$$
\hat \delta = r + \gamma  V_\phi(s') - V_\phi(s)
$$
and then use the (approximated) TD error to compute the policy gradient
 \begin{equation}
 \nabla_\theta J(\theta) = E \left[ \nabla_\theta log {\pi_\theta}(s,a) \hat \delta\right]
 \label{eq:gradA}
 \end{equation}
This approach only requires one set of critic parameters $\phi$
 
 
 \hl{-------------------------------------}
 




can be roughly categorized in two different families: Q-learning methods, and  policy-optimization methods.


In Q-learning methods, as Deep Q Network (DQN) \cite{mnih2013playing}, the agent learns an approximation $Q_\theta(\bm{s}, \bm{a})$ of the optimal action-value function $Q^\ast(\bm{s}, \bm{a})$, that is the value function when executing $\bm{a}$ in state $\bm{s}$ and then act according to $\pi$ for the rest of the training episode. The corresponding optimal policy $\pi^\ast$ is evaluated by choosing, in each state $\bm{s}$, the action $\bm{a}$ which maximizes $Q_\theta(\bm{s}, \bm{a})$. A DNN is commonly used for the estimated $Q_\theta$ In high-dimensional spaces or complex environments, hence the method name.

In policy-optimization methods, as policy-gradients ones, instead, the agent  attempt at directly learning the control policy $\pi(\bm{s})$ that maximize a performance index $J$.

Policy-gradient methods rely on an on-policy evaluation 


 works by running the current policy $\pi_{\theta_j}$ in $n_{env}$ independent realizations of the environment for $n_b$ training episodes \hl{each/each one}, and collecting a set of trajectories $\{ \tau_i\}_{i = 1, \dots, n_{env} n_b}$. 
 
 At the end of the sampling process, the policy performance are evaluated 
 
 by using a  performance index that has typically the form:

that is an \hl{unbias/biased yet low-variance}  estimated


\hl{controllare bene, non mi torna}
\begin{equation}
    J(\theta_j) =  \underset{\tau \sim \pi_{\theta_j}}{\mathbb{E}}\left[\sum_{k = 0}^{N} \log{\pi_{\theta_j}(\bm{a}_k | \bm{s}_k)} \hat{A}_{k}\right]
    \label{eq:Jvan}
\end{equation}




REINFORCE


 Eq. (XXX) is called the policy gradient and the form of this equation is referred
to as the REINFORCE method 

 it was shown that the reward $r k (x k , u k )$ in Eq. (18) can be replaced with state-
action value function $Q^\pi (x k , u k )$, this result is known as the Policy Gradient Theorem.


Furthermore, the variance of the policy gradient estimate that is derived from the Monte Carlo
roll-outs, $\tau^i$ , is reduced by subtracting a state-dependent baseline from $Q^\pi(x_k , u_k )$.

By choosing
is commonly chosen to be the state value function $V \pi (x k )$, and we can deﬁne
$A^\pi(x_k , u_k ) = Q^\pi (x_k, u_k ) - V^\pi (x_k)$. 

This method is known as the Advantage-Actor-Critic (A2C) Method.
The policy gradient for the A2C method is given by

$$ EQUAZIONE $$


SAC

the idea is to have two neural networks that run in parallel (as %in the \gncnet{} reported 
in Fig.~\ref{fig:gncnet}) and are concurrently updated: a (policy-based) Actor, that returns a parametrized policy $\pi_\theta$, and a (value-based) Critic, that returns an approximation of the on-policy value function $V_\phi$. So, the Actor controls the agent behavior while the Critic evaluates the agent performance and gives a feedback to the Actor in order to efficiently update the policy. The basic Actor-Critic RL scheme is reported in Fig.~\ref{fig:AC}.

==> RL low-thrust paper/PPO.tex <==


Policy-based RL

In an episodic environment, a natural measurement is the start value of the policy, which is the expected value of the start state:

$$J_1(\theta) = V_{\pi_\theta}(s_1) = E \pi \theta [v_1] $$


$$ E_{\tau \sim \pi_\theta} $$


PPO employs a clipped surrogate objective to prevent the new policy from straying away from the old one. The clipped objective function of state-action ($s_t$, $a_t$) is

Weighted combination of n-step returns
\begin{align}
   A_{GAE} = \sum_n {w_n \hat A_n^\pi (s_t, a_t)} \\
   w_n = \lambda^{n-1} \\
   %
   \hat A_{GAE} \sum_{t'=t}^N (\gamma \lambda)^{t'-t} \delta_{t'} \\
    \delta_{t'} = r(s_{t'}, a_{t'}) + \gamma \hat V_\phi^\pi(s_{t'+1}) - \hat V_\phi^\pi(s_{t'}) 
\end{align}

 



Policy gradient methods work by computing an estimator of the policy gradient and plugging it
into a stochastic gradient ascent algorithm. The most commonly used gradient estimator has the
form








A state-of-the-art policy gradient method named Proximal Policy Optimization~\cite{schulman2017proximal} is adopted in this paper because of the high performance demonstrated on a number of continuous and high-dimensional control problems.







Policy gradient methods works by running the current policy $\pi_{\theta_j}$ in $n_{env}$ independent realizations of the environment for $n_b$ training episodes \hl{each/each one}, and collecting a set of trajectories $\{ \tau_i\}_{i = 1, \dots, n_{env} n_b}$. At the end of the sampling process, the policy performance are evaluated by using a policy performance index that has typically the form:
\hl{controllare bene, non mi torna}
\begin{equation}
    J(\theta_j) =  \underset{\tau \sim \pi_{\theta_j}}{\mathbb{E}}\left[\sum_{k = 0}^{N} \log{\pi_{\theta_j}(\bm{a}_k | \bm{s}_k)} \hat{A}_{k}\right]
    \label{eq:Jvan}
\end{equation}
where $\tau = (\bm{s}_0, \bm{a}_0, \bm{s}_1, \bm{a}_1, \dots)$ represents a trajectory, $\pi_\theta(\bm{a}_k | \bm{s}_k)$ is a stochastic policy, that express the probability of taking action $\bm{a}_k$ in state $\bm{s}_k$, and $\hat{A}_k$ is an estimator of the advantage function, defined as:
\begin{equation}
    A^\pi(\bm{s}_k, \bm{a}_k) = Q^\pi(\bm{s}_k, \bm{a}_k) - V^\pi(\bm{s}_k)
\end{equation}
which expresses by how much the total reward improves by taking a specific action $\bm{a}_k$ in state $\bm{s}_k$ instead of randomly selecting the action according to $\pi_\theta(\cdot|\bm{s}_k)$.
From a computational point of view, the advantage function is usually approximated by using the so-called generalized advantage estimation:
\begin{align}
    \hat{A}_k &= \sum_{k'= k}^{N-1} (\gamma \lambda)^{k'-k} \delta_{k'} \\
    \delta_k &= r_k + \gamma V_\phi(\bm{s}_{k+1}) - V_\phi(\bm{s}_{k})
\end{align}

\hl{questa non la so, va controllata}
%\hl{delta dovrebbe essere qualcosa come temporal difference TD($\lambda$). Si dimostra che E[delta] = A.}

At this point, the policy parameters $\theta$ are updated via stochastic gradient ascent on that performance index:
\begin{equation}
    \theta_{j+1} = \theta_{j} + \alpha \nabla_\theta J(\theta)|_{\theta_j}
\end{equation}
where $\alpha$ indicates the learning rate, that usually is a decreasing function of the training step number.
In an analogous way, the value function parameters $\phi$ are updated via gradient descent on the mean-squared error $E(\phi)$ between the current estimate of value function and the rewards-to-go, that is:
\begin{equation}
    E(\phi) = \underset{\tau \sim \pi_{\theta}}{\mathbb{E}}\left[ \frac{1}{N} \sum_{k = 0}^{N} \left(V_\phi (\bm{s}_k) - \sum_{k' = k}^{N} r_{k'} \right)^2 \right]
\end{equation}

The problem with performance index \eqref{eq:Jvan} is that, empirically, it tends to perform too large policy updates, which are often the cause of performance collapse.
PPO was created with the aim of improving the stability of policy-gradient methods by avoid having too large policy updates. 
This is accomplished by using a so-called ``clipped surrogate objective function'' $J^{clip}$ in place of $J$, that constraints the updated policy $\pi_{\theta_j}$ to stay in a small range $\epsilon$, named clip range, around the previous value $\pi_{\theta_{j-1}}$, by clipping the probability that the new policy moves outside of interval $[1-\epsilon, 1+\epsilon]$.
So, by introducing a probability ratio
\hl{gli serve un simbolo migliore perche' $r$ lo abbiamo usato per il raggio}:
\begin{equation}
    r_k(\theta_j) = \frac{\pi_{\theta_j}(\bm{a}_k | \bm{s}_k)}{\pi_{\theta_{j-1}}(\bm{a}_k | \bm{s}_k)}
\end{equation}
the clipped objective function can be written as:
\begin{equation}
    J^{clip}(\theta_j) =  \underset{\tau \sim \pi_{\theta_j}}{\mathbb{E}}\left[ \frac{1}{N} \sum_{k = 0}^{N}  \min{\left( r_k(\theta_j) \hat{A}_k, \mbox{clip}(r_k(\theta_j), 1-\epsilon, 1+\epsilon) \hat{A}_k\right)} \right]
\end{equation}
In the same fashion as the learning rate, also the clip range $\epsilon$ can be a decreasing function of the training step number.
Typically, in PPO the policy and value-function update is done all at once by gathering in the set of parameters $\theta$ the weights and biases of both the actor and critic networks, and including the value function error term $E$ in the objective function. Eventually, an entropy term $S$ is added to ensure sufficient exploration, bringing to the final surrogate objective function:
\begin{equation}
    J^{ppo}(\theta_j) = J^{clip}(\theta_j) - c_1 E(\theta_j) + c_2 S(\theta_j)
\end{equation}
where $c_1$ and $c_2$ are two hyperparameters named value function coefficient and entropy coefficient, respectively.
Moreover, with respect to classical policy gradient methods, in PPO the policy update is performed by running $n_{opt}$ epochs of stochastic gradient descent over $n_b$ sampling mini-batches, each with $n_{env}N$ training samples.
The algorithm terminates after a total number of training steps equal to $M$.

As a final remark, it is worth noting that the RL algorithm just presented is completely model-free, as it does not depend in any way on the mathematical form of the transition function $f$, control model $g$ and observation model $h$, nor on the expression of the probability distributions $P$.



\section{SCARTI}



\subsection{\hl{--------------------}}

 


 







Reducing Variance Using a Baseline

We subtract a baseline function B(s) from the policy gradient
This can reduce variance, without changing expectation


A good baseline is the state value function $B(s) = V^{\pi_\theta}(s)$

So we can rewrite the policy gradient using the advantage
function 
$$A^{\pi_\theta} = Q^{\pi_\theta}(s, a) - V^{\pi_\theta}(s)$$


For the true value function $V^{\pi_\theta}(s)$, the TD error $\delta^{\pi_\theta}$ is

$$\delta^{\pi_\theta} = r + \gamma V^{\pi_\theta}(s') - V^{\pi_\theta}(s)$$

is an unbiased estimate of the advantage function, that is $E_{\pi_\theta}[\delta^{\pi_\theta}] = A^{\pi_\theta}(s,a)$.

In practice we can use an approximate TD error
$$
\hat \delta = r + \gamma  V_\phi(s') - V_\phi(s)
$$
and then use the (approximated) TD error to compute the policy gradient
 $$
 \nabla_\theta J(\theta) = E \left[ \nabla_\theta log {\pi_\theta}(s,a) \hat \delta\right]
 $$

This approach only requires one set of critic parameters $\phi$






 


%While Monte Carlo methods only adjust their estimates once the final outcome is known, TD methods adjust predictions to match later, more accurate, predictions about the
% TD method bases its update in part on an existing estimate,
%we say that it is a bootstrapping method
%$$ g =\mathbb{E} \left[\nabla_\theta \log \pi_\theta(s, a)  \mathbb{E} \sum_{t' = t}^N r_{t'}-b(s_t) \right] $$
%
%Combining these two improvement one has $g =\mathbb{E} \left[\nabla_\theta \log \pi_\theta(s, a)  \hat A(s_t, a_t) \right] $











proximal policy optimization (PPO) simplifies Trust region policy optimization (TRPO) (Schulman, et al., 2015) 
 using a clipped surrogate objective while retaining similar performance.








The goal is thus to chose $\theta$ 

The value of the reward (objective) function depends on this policy and then various algorithms can be applied to optimize $\theta$ for the best reward.



In high-dimensional spaces or complex environments,






the agent  attempt at  learning the control policy $\pi(\bm{s})$ .
instead of learning the (e.g., Deep Q Network, DQN)




model-free RL approaches dos not rely on an \textit{a-priori} knowledge of the transition function $f$, control model $g$, and observation model $h$, nor of the probability distributions of disturbance $P$ (see Eq.s~\eqref{eq:MDP}-\eqref{eq:MDP2}) and work even in case these function are non-analytical.
\hl{questo e' utile per questo problema perche'}




 

 \hl{-------------------------------------}
 















 \hl{-------------------------------------}
The environment initializes an episode by randomly generating an internal state, mapping this
internal state to an observation, and passing the observation to the agent.

 At each step of the episode, an observation is generated from
the internal state and given to the agent. The agent uses this observation to generate
an action that is sent to the environment; the environment then uses the action and the
current state to generate the next state and a scalar reward signal. The reward and the
observation corresponding to the next state are then passed to the agent



 
 
  The DNNs can be Feedforward Networks (FNNs), as Multi-Layer Perceptron (MLP) networks, as well as recurrent networks, as Long-Short Term Memory (LSTM) networks. 
  
  
 
 n this context, the term \gncnet{} (namely, Guidance and Control Network) was coined at the European Space Agency \cite{izzo2019survey} to refer to a Deep Neural Network (DNN) used to map any observation $\bm{o}_k$ of the spacecraft state $\bm{s}_k$ (e.g., position, velocity and mass) to the corresponding (parameterized) policy $\pi_\theta(\bm{s}_k)$ (e.g., the thrust vector) and/or (parameterized) value function $V_\phi(\bm{s}_k)$.
%, that is, the overall performance score that is expected by following the optimal policy starting from that state
 
 The computational effort is mainly spent on the network training, which has to be performed just once. After training, the \gncnet{} can be used to evaluate an optimal state-feedback control policy at almost no computational cost. This feature makes the \gncnet{} also suitable to be used as an integrated on-board guidance and control system during the cruise phase of interplanetary missions, providing the spacecraft with the capability of autonomously adjusting its trajectory in situations where corrective commands from Earth are not possible, such as during a short-duration maneuver (e.g., the flyby of an asteroid) or when the number of available radio links with Earth is limited. Furthermore, the trained network is able to run also on cheaper processors, as those typically mounted on-board of micro-spacecraft because of the limited budget.
 
 
 
 

 
 
 
 
 \hl{---------------------------------}
 



In order to avoid having a third DNN,
the 

One may easily prove that

the TD error $\delta^{\pi_\theta} = r + \gamma V^{\pi_\theta}(s') - V^{\pi_\theta}(s)$ is
is an unbiased estimate of the advantage function, that is $E_{\pi_\theta}[\delta^{\pi_\theta}] = A^{\pi_\theta}(s,a)$.
Hence,



For the true value function $V^{\pi_\theta}(s)$, the TD error $\delta^{\pi_\theta}$ is


In practice we can use an approximate TD error
$$
\hat \delta = r + \gamma  V_\phi(s') - V_\phi(s)
$$
and then use the (approximated) TD error to compute the policy gradient
 \begin{equation}
 \nabla_\theta J(\theta) = E \left[ \nabla_\theta log {\pi_\theta}(s,a) \hat \delta\right]
 \label{eq:gradA}
 \end{equation}
This approach only requires one set of critic parameters $\phi$
 
 
 \hl{-------------------------------------}
 




can be roughly categorized in two different families: Q-learning methods, and  policy-optimization methods.


In Q-learning methods, as Deep Q Network (DQN) \cite{mnih2013playing}, the agent learns an approximation $Q_\theta(\bm{s}, \bm{a})$ of the optimal action-value function $Q^\ast(\bm{s}, \bm{a})$, that is the value function when executing $\bm{a}$ in state $\bm{s}$ and then act according to $\pi$ for the rest of the training episode. The corresponding optimal policy $\pi^\ast$ is evaluated by choosing, in each state $\bm{s}$, the action $\bm{a}$ which maximizes $Q_\theta(\bm{s}, \bm{a})$. A DNN is commonly used for the estimated $Q_\theta$ In high-dimensional spaces or complex environments, hence the method name.

In policy-optimization methods, as policy-gradients ones, instead, the agent  attempt at directly learning the control policy $\pi(\bm{s})$ that maximize a performance index $J$.

Policy-gradient methods rely on an on-policy evaluation 


 works by running the current policy $\pi_{\theta_j}$ in $n_{env}$ independent realizations of the environment for $n_b$ training episodes \hl{each/each one}, and collecting a set of trajectories $\{ \tau_i\}_{i = 1, \dots, n_{env} n_b}$. 
 
 At the end of the sampling process, the policy performance are evaluated 
 
 by using a  performance index that has typically the form:

that is an \hl{unbias/biased yet low-variance}  estimated


\hl{controllare bene, non mi torna}
\begin{equation}
    J(\theta_j) =  \underset{\tau \sim \pi_{\theta_j}}{\mathbb{E}}\left[\sum_{k = 0}^{N} \log{\pi_{\theta_j}(\bm{a}_k | \bm{s}_k)} \hat{A}_{k}\right]
    \label{eq:Jvan}
\end{equation}




REINFORCE


 Eq. (XXX) is called the policy gradient and the form of this equation is referred
to as the REINFORCE method 

 it was shown that the reward $r k (x k , u k )$ in Eq. (18) can be replaced with state-
action value function $Q^\pi (x k , u k )$, this result is known as the Policy Gradient Theorem.


Furthermore, the variance of the policy gradient estimate that is derived from the Monte Carlo
roll-outs, $\tau^i$ , is reduced by subtracting a state-dependent baseline from $Q^\pi(x_k , u_k )$.

By choosing
is commonly chosen to be the state value function $V \pi (x k )$, and we can deﬁne
$A^\pi(x_k , u_k ) = Q^\pi (x_k, u_k ) - V^\pi (x_k)$. 

This method is known as the Advantage-Actor-Critic (A2C) Method.
The policy gradient for the A2C method is given by

$$ EQUAZIONE $$


SAC

the idea is to have two neural networks that run in parallel (as %in the \gncnet{} reported 
in Fig.~\ref{fig:gncnet}) and are concurrently updated: a (policy-based) Actor, that returns a parametrized policy $\pi_\theta$, and a (value-based) Critic, that returns an approximation of the on-policy value function $V_\phi$. So, the Actor controls the agent behavior while the Critic evaluates the agent performance and gives a feedback to the Actor in order to efficiently update the policy. The basic Actor-Critic RL scheme is reported in Fig.~\ref{fig:AC}.

==> RL low-thrust paper/RL.tex <==

This section briefly outlines the mathematical framework of the RL method
%of deep reinforcement fearning, 
selected to tackle the problem outlined in the previous section.
%
The RL algorithm adopted in this work is \textit{Proximal Policy Optimization}~\cite{schulman2017proximal}, which is a model-free policy-gradient actor-critic method, widely recognized for the high performance demonstrated on a number of continuous and high-dimensional control problems.

A model-free approach is particularly suited to design a robust trajectory. In fact, model-free RL methods do not rely on an \textit{explicit} knowledge of the MDP (Eqs.~\eqref{eq:MDP}-\eqref{eq:MDP2}) for returning the optimal control policy $\pi^\ast$.
This fact leaves us the freedom to use complex, and possibly non-analytical,
expressions for the transition function $f$, control model $g$, observation model $h$, and/or disturbance distributions, without requiring any change in the algorithm.
 

Policy-gradient algorithms are a common choice in RL.
The underlying idea is to directly learn the policy $\pi(\bm{s})$ that maximizes the performance index $J$. %rather than looking for the  optimal action-value function $Q^\ast(\bm{s}, \bm{a})$, as in Q-learning methods\cite{mnih2013playing} and found the policy by \hl{looping/working}.
A stochastic policy is generally considered, as more robust and oriented toward exploration than deterministic ones.
In this sense, 
$\pi(\bm{s})$ should be intended as a shorthand for $\pi(\bm{a} | \bm{s})$, that is, the probability of choosing action $\bm{a}$, conditioned by being the system in the state $\bm{s}$.
%\hl{Although any probability distribution can be used, in practice the policy is often Gaussian and the network actually outputs the mean and variance of the underlying Gaussian distribution.}

In order to cope with complex environments and possibly large (and continuous) state and/or action spaces,  the policy $\pi$ is usually modeled by a DNN {with} parameters (i.e., weights and biases) $\theta$, and referred to as $\pi_\theta(\bm{a} | \bm{s})$ to make the dependence on the network parameters explicit.
%
A typical DNN is composed by a sequence of \textit{layers}, each made up of a number of basic units, called \textit{neurons}. 
A Multi-Layer Perceptron (MLP) is adopted in the present work:
each neuron receives input signals from the units in the previous layer, generates an output signal as a linear combination of the inputs, elaborated through a (typically nonlinear) \textit{activation function}, and sends this signal to the units in the next layer.
% The first layer, or input layer, receives as input a given set of values for the function inputs; the final layer, or output layer, returns an estimate of the corresponding function outputs.
More complex architectures, such as Recurrent Neural Networks (RNNs), are also used in deep RL to cope with partially-observable or non-Markov environments, but they are not considered in this work.
%The computational effort is mainly spent on the network training, which has to be performed just once. After that, the DNN can be used to approximate the function outputs, for any given set of inputs, at almost no computational cost.
%\hl{NN - fine}
%
In the case of a deterministic policy, 
the network directly outputs the action, given the current system state as input; instead, when a stochastic policy is considered, the network returns some parameters 
of the underlying probability distribution,
such as mean and variance for a Gaussian distribution, which is the most frequently adopted.
The actual action is then sampled from this probability distribution.

Once the network architecture (i.e., number of layers, layer density, and activation functions) is assigned, the problem reduces to the search of the parameters $\theta^\ast$ that maximize the merit index $J$:
\begin{equation}
\theta^\ast = \mbox{arg} \max_\theta J(\theta) = \mbox{arg} \max_\theta \left( \underset{\tau\sim \pi_\theta}{\mathbb{E}} \left[\sum_{k=0}^{N-1} r_k \right] \right)
\label{eq:grad_pol}
\end{equation}
where $r_k = R(\bm{s}_k, \bm{u}_k, \bm{s}_{k+1})$ is the immediate reward collected after taking action $\bm{a}_k \sim \pi_\theta( \cdot | \bm{s}_k)$.



In order to solve Eq.~\eqref{eq:grad_pol}, policy-gradient algorithms perform a (stochastic) gradient ascent update on $\theta$, that is: $\theta \leftarrow \theta + \alpha \nabla_\theta J(\theta)$,
where $\alpha$ is the \textit{learning rate}, which is a constant, or slowly decreasing, user-defined hyper-parameter that controls the step-size of the gradient update. 



The \textit{Policy Gradient Theorem}~\cite{sutton2018reinforcement} is used to rewrite the gradient $\nabla_\theta J(\theta)$ in a more suitable form:
\begin{equation}
    \nabla_\theta  J(\theta) = \underset{\tau\sim \pi_\theta}{\mathbb{E}} \left[ \sum_{k=0}^{N-1} \nabla_\theta \log \pi_\theta(\bm{a}_k | \bm{s}_k)\,  Q^{\pi_\theta}(\bm{s}_k,\bm{a}_k) \right]
    \label{eq:nablaJ}
\end{equation}
where $Q^{\pi_\theta}(\bm{s},\bm{a}) = \mathbb{E}_{\tau \sim \pi_\theta} 
\left[\sum_{k'=k}^{N-1} r_{k'}\, |\, \bm{s}_k = \bm{s}, \bm{a}_k = \bm{a} \right]$ is the Action-Value function, or simply Q-function, that is, the expected return obtained by starting in state $\bm{s}$, taking action $\bm{a}$ and then acting according to $\pi_\theta$.
%Qw(.) is a action value function parameterized by w


%$$ g =\mathbb{E} \left[\nabla_\theta \log \pi_\theta(s, a)  \mathbb{E} Q^\pi(s_t,a_t) \right] $$

%%%%%%%%%%%%%%%%%%%%%%%%
%\hl{[OPZIONALE]}  The Q-value function $Q^\pi(s_t,a_t)$ can be estimated by Monte-Carlo methods using the the mean return over episode samples, that is 
%$$Q^\pi(s_t,a_t) \approx  \mathbb{E} G_t =  \mathbb{E} \sum_{t' = t}^N r_{t'}$$
%hence \begin{equation}
%g =\mathbb{E} \left[\nabla_\theta \log \pi_\theta(s, a)  \mathbb{E} \sum_{t' = t}^N r_{t'} \right] 
%\label{eq:REINFORCE}
%\end{equation} 
%Eq.~\eqref{eq:REINFORCE} is at the basis of the REINFORCE algorithm~\hl{ref}.
%\hl{FINE}
%%%%%%%%%%%%%%%%%%%




The Q-function might be estimated by a Monte-Carlo approach, using the average return over episode samples. While unbiased, this estimate has a high variance, which makes this approach unsuitable for practical purposes.
%
An improved solution relies on approximating the Q-value function by a second DNN, leading to the so called Actor-Critic method.
%
The two neural networks run in parallel and are concurrently updated:
the Actor, which returns the parametrized policy $\pi_\theta$, is updated by gradient ascent on the policy-gradient;
the Critic, which returns the parametrized Q-function $Q_\phi$,
is recursively updated using Temporal Difference~\cite{sutton2018reinforcement}.
%
Intuitively, the Actor controls the agent behavior while the Critic evaluates the agent performance and gives a feedback to the Actor in order to efficiently update the policy. 

To further improve the stability of the learning process and reduce variance in the sample estimate for the policy gradient, it is possible to subtract a function of the system state only, called baseline $b(\bm{s})$, from the expression~\eqref{eq:nablaJ} of the policy gradient, without changing it in expectation.
The most common choice of baseline is the value function $V^{\pi_\theta}(\bm{s})$, which, subtracted from the Action-Value function $Q^{\pi_\theta}(\bm{s},\bm{a})$, leads to the definition of the advantage function $A^{\pi_\theta}(\bm{s},\bm{a}) = Q^{\pi_\theta}(\bm{s},\bm{a}) - V^{\pi_\theta}(\bm{s})$, which expresses by how much the total reward improves by taking a specific action $\bm{a}$ in state $\bm{s}$, instead of randomly selecting the action according to $\pi_\theta(\cdot|\bm{s})$.
%
From a computational point of view, the advantage function is usually computed by using the so-called generalized advantage estimation:
\begin{equation}
    \hat{A}_{k} = \sum_{k'= k}^{N-1} (\gamma \lambda)^{k'-k} \delta_{k'}
    \label{eq:advantage}
\end{equation}
where: 
\begin{equation}
   \delta_k = r_k + \gamma V^{\pi_\theta}(\bm{s}_{k+1}) - V^{\pi_\theta}(\bm{s}_{k}) 
   \label{eq:TDerror}
\end{equation}
is the Temporal-Difference error, that is an unbiased estimate of the advantage function, being ${\mathbb{E}}_{\tau \sim \pi_\theta}[\delta_k] = A^{\pi_\theta}(\bm{s}_k,\bm{a}_k)$.

So, the policy gradient can be evaluated as:
\begin{equation}
    \nabla_\theta  J(\theta) = \underset{\tau\sim \pi_\theta}{\mathbb{E}} \left[ \sum_{k=0}^{N-1} \nabla_\theta \log \pi_\theta(\bm{a}_k | \bm{s}_k)\,  \hat{A}_{k} \right]
    \label{eq:nablaJ_A}
\end{equation}

This leads to the Advantage Actor-Critic (A2C) method \cite{mnih2016asynchronous}, whose basic architecture is reported in Fig.~\ref{fig:AC}. In this case, the Critic returns a parameterized value function $V_\phi$, necessary for the advantage estimation in Eqs.~\eqref{eq:advantage}--\eqref{eq:TDerror}.
\begin{figure} [htb]
    \centering
    \includegraphics[width = 0.6\textwidth]{Figures/AC.pdf}
    \caption{Schematic of the Advantage Actor-Critic RL process, for a deterministic MDP.}
    \label{fig:AC}
\end{figure}






PPO can be seen as a further evolution of the (advantage) Actor-Critic  method.
In order to avoid too large policy updates when using Eq.~\eqref{eq:nablaJ_A} during gradient ascent, which usually cause performance collapse, PPO introduces a ``clipped surrogate objective function'' $J^{clip}$ in place of $J$, to constrain the updated policy $\pi_{\theta}$ to stay in a small range $\epsilon$, named clip range, around the previous value $\pi_{\theta_{old}}$, by clipping the probability that the new policy moves outside of the interval $[1-\epsilon, 1+\epsilon]$.

Let $\tilde{r}_k(\theta)$ be the probability ratio:
\begin{equation}
    \tilde{r}_k(\theta) = \frac{\pi_{\theta}(\bm{a}_k | \bm{s}_k)}{\pi_{\theta_{old}}(\bm{a}_k | \bm{s}_k)}
\end{equation}
The clipped surrogate objective function can be written as:
\begin{equation}
    J^{clip}(\theta) =  \underset{\tau \sim \pi_{\theta}}{\mathbb{E}}\left[ \frac{1}{N} \sum_{k = 0}^{N-1}  \min{\left( \tilde{r}_k(\theta) \hat{A}_k, \mbox{clip}(\tilde{r}_k(\theta), 1-\epsilon, 1+\epsilon) \hat{A}_k\right)} \right]
\end{equation}

%In the same fashion as the learning rate, also 
Empirical evidences suggest that using a clip range $\epsilon$ that decreases linearly with the training steps improves the learning effectiveness.
Typically, in PPO the policy and value function updates are carried out all at once by gathering in the set of parameters $\theta$ the weights and biases of both the Actor and Critic networks, and by including  in the objective function a mean-squared value function error term $H$:
\begin{equation}
    H(\theta) = \underset{\tau \sim \pi_{\theta}}{\mathbb{E}}\left[ \frac{1}{N} \sum_{k = 0}^{N-1} \frac{1}{2} \left(V_\theta (\bm{s}_k) - \sum_{k' = k}^{N} r_{k'} \right)^2 \right]
\end{equation}
and an entropy term $S$:
\begin{equation}
S(\theta) = \underset{\tau \sim \pi_{\theta}}{\mathbb{E}}\left[ \frac{1}{N} \sum_{k = 0}^{N-1} \mathbb{E}_{ 
\bm{a} \sim \pi_\theta(\cdot| \bm{s}_k)} \left[ - \log{ \pi_\theta(\bm{a} | \bm{s}_k)} \right]  \right]
\end{equation}
which is usually added to ensure sufficient exploration, and prevent premature convergence to a suboptimal deterministic policy \cite{mnih2016asynchronous}. 
Eventually, the final surrogate objective function is:
\begin{equation}
    J^{ppo}(\theta) = J^{clip}(\theta) - c_1 H(\theta) + c_2 S(\theta)
\end{equation}
where
$c_1$ and $c_2$ are two hyper-parameters, named value function coefficient and entropy coefficient, that control the relative importance of the various terms. 
%where
%$ S(\theta) = - \mathbb{E}_{a \sim \pi_\theta(\cdot| \bm{s}_k)} \left[ \pi_\theta(\bm{a} | \bm{s}_k) \log{ \pi_\theta(\bm{a} | \bm{s}_k)} \right] $
%is and entropy regularization term, introduced to prevent premature convergence to a deterministic policy,
%is a mean-squared-error loss function
%averaged ...
%and $c_1$ and $c_2$ are two hyper-parameters, named value function coefficient and entropy coefficient, that control the relative importance of these two terms. 
 
The overall learning process consists of two well-distinguished phases that are repeated iteratively:
i) \textit{policy rollout}, 
during which the current policy $\pi_{\theta}$ is run
in $n_{env}$ independent (e.g. parallel) realizations of the environment for $n_b$ training episodes, collecting a set of $n_{env} n_b$  trajectories $\tau^i$; 
ii) \textit{policy update}, 
%\hl{a stochastic gradient descent is performed to update the network parameters}
which is performed by running $n_{opt}$ epochs of stochastic gradient ascent over $n_b$ sampling mini-batches
of on-policy data, that is, the data coming from the last rollout only.
The algorithm terminates after a total number of training steps equal to $T$.
 


 

%Moreover, with respect to classical policy-gradient methods, in PPO the policy update is performed by running $n_{opt}$ epochs of stochastic gradient descent over $n_b$ sampling mini-batches, each with $n_{env}N$ training samples. The algorithm terminates after a total number of training steps equal to $T$.


\subsubsection{Remark.} 
The above described framework has been derived in case of a (perfectly observable) Markov Decision Process.
When a perfect knowledge of the state is not available
or when the observations differ from the state, the same RL algorithm can be used, but in this case the Actor and Critic networks take as an input directly the observation $\bm{o}_k$.
%and outputs both the action probability $\pi_\theta(\bm{o}_k)$


\subsection{Implementation Details}%
The results presented in this work have been obtained by using the PPO algorithm implementation by Stable Baselines \cite{stable-baselines2018}, an open-source library containing a set of improved implementations of RL algorithms based on OpenAI Baselines.
The scientific library \textit{pykep}\cite{izzo2012pykep}, developed at the European Space Agency, was instead used for the astrodynamics routines.


The selected \gncnet{} consists of two separate head networks, one for the control policy and the other for the value function, each one composed of two hidden layers. The \gncnet{} architecture is summarized in Table~\ref{tab:net}, which reports the number of neurons in each layer and the activation function used in each neuron.
The tuning of PPO hyper-parameters was performed by using Optuna~\cite{optuna2019}, an open source hyper-parameter optimization framework for automated hyper-parameter search. The hyper-parameter optimization was realized on a deterministic version of the RL environment, with a budget of 500 trials, each with a maximum of $\SI{3e5}{}$ training steps. The optimal value of the hyper-parameters used in all simulations is reported in Table~\ref{tab:hyper}.


%with a shared network place btween the input layer and the two head

%Optionally, a shared DNN is placed before the two head networks. Parameters $\theta$ and $\phi$ indicate the parameters (i.e., weights and biases) of the network used for the policy and value function approximation, respectively. 
%/ 
%Also it was empirically shown that using a partially network between Actor and Critic reduce the overall number of parameters to train, hence speed up training process.









%\begin{figure} [htb]
%    \centering
%    \includegraphics[width = 0.7\textwidth]{Figures/GCNet.pdf}
%    \caption{Generic \gncnet{}, composed by a shared network, a policy network and a value function network. \hl{la rete input the observation and outputs ...} }
%    \label{fig:gncnet}
%\end{figure}


\begin{table}[!htb]
%   \resizebox{10cm}{!}{
     \begin{minipage}{.45\textwidth}
        \centering
        \caption{Network Configuration.}\label{tab:net}
        \centering
        \begin{tabular}{c  c c} % Column formatting, 
          \hline 
           & Policy  & Value \\
          & network & network\\
           \hline 
          Layer 1 & 64 & 64\\
          %\hline
          Layer 2 & 64 & 64\\
          %\hline
          Output & 3 & 1 \\
         % \hline
          Activation & tanh & tanh \\
          \hline 
       \end{tabular} 
    \end{minipage}
    \hfill
    \begin{minipage}{.45\textwidth}
    \begin{threeparttable}
             \caption{PPO hyperparameters.} \label{tab:hyper}
        \centering
       \begin{tabular}{c c} % Column formatting, 
          \hline 
          Hyper-parameter  & Value\\
          \hline
          $\gamma$       & $0.9999$ \\
          $\lambda$ & $0.99$ \\
          $\alpha$     &  $2.5 \times 10^{-4} \left(1 - {t}/{T} \right)$\tnote{$\star$} \\
          $\epsilon$ &  $0.3 \left(1 - {t}/{T}\right)$\tnote{$\star$} \\
          $c_1$  &  $0.5$ \\
          $c_2$ & $4.75 \times 10^{-8}$ \\
          $n_{opt}$ & $30$\\
          \hline
          %\multicolumn{2}{r}{$t$ indicates the training step number} \\
          %\multicolumn{2}{r}{$T$ the total number of training steps.}
       \end{tabular}
       \begin{tablenotes}\footnotesize
        \item [$\star$] $t$ indicates the training step number
        %$T$ the total number of training steps.
        \end{tablenotes}
       \end{threeparttable}
    \end{minipage}%
%
%}  
\end{table}

When dealing with constrained optimization problems, constraint violations are typically included as penalty terms inside the reward function (see Eq.~\eqref{eq:rew}). In these cases, a penalty-based $\varepsilon$-constraint method, similar to those sometimes used in stochastic global optimization \cite{federici2020eos}, proved to be helpful to enforce constraints more gradually during optimization, allowing the agent to explore to a greater extent the solution space  at the beginning of the training process.
 %
For this reason, as a modest original contribution of this paper, the constraint satisfaction tolerance $\varepsilon$ also varies during the training, according to a (piecewise constant) decreasing trend:
\begin{equation}
\varepsilon = 
    \begin{cases}
    0.01 & \mbox{for the first } T/2  \mbox{ training steps}\\
    0.001 & \mbox{for the second } T/2  \mbox{ training steps}
    \end{cases}
\end{equation}
















 




  
 

























==> RL low-thrust paper/Tables/tab-1.tex <==
\begin{table}[htbp]
	%\fontsize{10}{10}\selectfont
    \caption{Problem data.}
   \label{tab:data}
        \centering 
   \begin{tabular}{c c} % Column formatting, 
      \hline 
      Variable  & Value\\
      \hline 
      $N$       & 40 \\
      $t_f,\, \si{days}$     &  $358.79$ \\
      $T_{max},\, \si{\kilo\newton}$ &  $0.50$ \\
      $u_{eq},\, \si{\kilo\meter/\second}$  &  $19.6133$ \\
      $m_0,\, \si{\kilo\gram}$ & $1000$ \\
      $\mu_\Sun,\,  \si{\kilo\meter^3/\second^2}$ & $132712440018$ \\
      $\bm{r}_\Earth,\, \si{\kilo\meter}$ & $[-140699693,\, -51614428,\, 980]^T$\\
      $\bm{v}_\Earth,\, \si{\kilo\meter/\second}$ & $[9.774596,\, -28.07828,\, 4.337725 \times 10^{-4}]^T$\\
      $\bm{r}_\Mars,\, \si{\kilo\meter}$ & $[-172682023,\, 176959469,\, 7948912]^T$\\
      $\bm{v}_\Mars,\,\si{\kilo\meter/\second}$ & $[-16.427384,\, -14.860506,\, 9.21486 \times 10^{-2}]^T$\\
      \hline
   \end{tabular}
\end{table}



==> RL low-thrust paper/Tables/tab-MC.tex <==
\begin{table}[!h]
%\fontsize{10}{10}\selectfont
    \caption{Results of the Monte Carlo simulations in terms of mean value (mean), standard deviation (std), and success rate (SR).}
\begin{adjustwidth}{-1in}{-1in}% adjust the L and R margins by 1 inch
   \label{tab:MC}
        \centering 
    %{\renewcommand{\arraystretch}{1.2}
   \begin{tabular}{l  c c   c c   c c  c } % Column formatting, 
      \hline 
      \multirow{2}{*}{Policy} & \multicolumn{2}{c }{$m_f,\,\,\si{\kilo\gram}$} & \multicolumn{2}{c }{$\Delta r_f/r_\Mars,\,\,$\textperthousand}  & \multicolumn{2}{c }{$\Delta v_f/v_\Mars,\,\,$\textperthousand} & \multirow{2}{*}{SR, \%}  \\%  & \multicolumn{2}{c}{$J$}  \\
       & mean  & std &  mean & std &  mean & std &  \\%  &  mean & std \\
      \hline 
      $\pi^{st}$ & $578.04$ & $9.48$ & $0.742$ & $0.322$ & $0.0403$ & $0.211$ & $80.0$ \\% & $-0.4249$ & $0.0148$ \\
      %\hline 
      $\pi^{obs}$ & $580.94$ & $9.53$ & $0.807$ & $0.343$ & $0.0502$ & $0.299$ & $70.6$ \\% & $-0.4234$ & $0.0147$ \\
      %\hline
     $\pi^{ctr}$ & $591.13$ & $0.685$ & $0.846$ & $0.426$ & $0.0620$ & $0.270$ & $69.0$ \\% & $-0.4161$ & $0.0330$ \\
      %\hline
     $\pi^{mte,1}$ & $579.02$ & $4.44$ & $0.980$ & $0.667$ & $0.0987$ & $0.438$ & $69.8$ \\% & $-0.4329$ & $0.0301$ \\
      %\hline
      $\pi^{mte,2}$ & $557.32$ & $4.77$ & $1.266$ & $2.048$ & $0.645$ & $3.451$ & $70.4$ \\% & $-0.4961$ & $0.195$ \\
      \hline
   \end{tabular}
   %}
  \end{adjustwidth}
\end{table}


==> RL low-thrust paper/Tables/tab-robust.tex <==
\begin{table}[!htbp]
	%\fontsize{10}{10}\selectfont
    \caption{Robust trajectory overview.    %, when trained by considering different types of uncertainties in the environment.
    }
   \label{tab:nom}
        \centering 
    %{\renewcommand{\arraystretch}{1.2}
   \begin{tabular}{l c c c | c c c c} % Column formatting, 
   \hline 
     \multirow{2}{*}{Policy} &\multicolumn{3}{c|}{Settings} & \multicolumn{4}{c}{Results} \\
      %\hline 
      & $T$ & $n_{env}$ & $n_b$ & $m_f,\,\,\si{\kilo\gram}$ & $\Delta r_f/r_\Mars,\,\,$\textperthousand  & $\Delta v_f/v_\Mars,\,\,$\textperthousand & $J$  \\
      \hline 
      $\pi^{unp}$& $48M$ & $8$ & $4$ & $600.23$ & $0.999$ & $0$ & $-0.3998$ \\
      $\pi^{st}$ & $112M$ & $8$ & $4$ & $588.41$ & $0.767$ & $0$ & $-0.4116$ \\
      $\pi^{obs}$& $200M$ & $8$ & $4$ & $591.48$ & $0.782$ & $0$ & $-0.4085$ \\
      $\pi^{ctr}$& $128M$ & $16$ & $4$ & $591.40$ & $0.814$ & $0$ & $-0.4086$ \\
      $\pi^{mte,1}$& $80M$ & $16$ & $4$ & $575.98$ & $3.689$ & $0$ & $-0.5585$ \\
      $\pi^{mte,2}$& $128M$ & $16$ & $8$ & $555.87$ & $2.273$ & $0$ & $-0.5078$ \\
      \hline 
   \end{tabular}
   %}
\end{table}

==> RL low-thrust paper/Tables/tab-unpMC.tex <==
\begin{table}[!htbp]
	%\fontsize{10}{10}\selectfont
    \caption{Performance of policy $\pi^{unp}$ in terms of satisfaction ratio, that is number of cases where the terminal constraints on final position and velocity are respected out of 500 runs, when deployed in %applied to
    various perturbed (stochastic) environments.
    }
   \label{tab:unpMC}
        \centering 
    {\renewcommand{\arraystretch}{1.2}
   \begin{tabular}{l  r r } % Column formatting, 
   \hline 
   \multirow{2}{*}{Perturbation} & \multicolumn{2}{c}{Success rate [\%]} \\
    & Position constraint & Velocity constraint \\
     %Perturbation & $\Delta r_f/r_\Mars$  SR [\%] & $\Delta v_f/v_\Mars$  SR [\%] \\
    % & SR [\%] & SR [\%] \\
      \hline 
      state & $0.0$  & $50.2$  \\
      observations & $0.0$ & $45.8$\\
      control &  $12.8$ & $64.4$\\
      single MTE & $18.8$ & $35.0$\\
      multiple MTEs & $16.8$ & $33.8$\\
      \hline 
   \end{tabular}
   }
\end{table}

%        r     v
%state : 0   50.2
%observation: 0 45.8
%control: 12.8 64.4
%MTE:  18.8 35.0
%MTEs: 16.8 33.8

==> RL low-thrust paper/results.tex <==

This section presents some %numerical results
preliminary results obtained by training the \gncnet{} on different environments (that is, mission scenarios), generated by considering separately each uncertainty source defined in the problem statement.
%
In order to validate the proposed approach, the solution found in a (deterministic) unperturbed scenario is compared with the optimal one provided by an indirect technique.
Then, the robustness and optimality of the obtained control policies is assessed by means of Monte Carlo campaigns performed in the considered uncertain scenarios. 
 


%\hl{The analysis of multiple/cross effects is left to future investigations}.
 
\subsection{Deterministic Optimal Trajectory}
The ability of the presented methodology to deal with traditional, deterministic, optimal control problems is investigated first, by comparing the solution provided by the control policy $\pi^{unp}$ trained in the deterministic (unperturbed) environment (see Eq.~\eqref{eq:dyn_kep}), 
%referred to training in the unperturbed environment, 
with the solution of the original Earth-Mars low-thrust transfer problem, found by using a well-established indirect optimization method used by the authors in other interplanetary transfers \cite{colasurdo2014tour}.
%
The two solutions are very close to each other in terms of trajectory and control direction.
Also, the final mass of the RL solution ($\SI{600.23}{kg}$) is in good agreement with the (true) optimal mass obtained by the indirect method ($\SI{599.98}{\kilo\gram}$).
This slight difference is partly due to the fact that RL satisfies the terminal constraints with a lower accuracy  ($10^{-3}$ in RL vs $10^{-9}$ in the indirect method), and partly due to the (approximated) time-discrete, impulsive dynamical model adopted in the MDP transcription.
%
%\hl{This high-quality result was obtained without any specific reward shaping,  unlike previous work in the literature.} \cite{portland2019Stanford}


%\hl{However, these results confermano che va tutto bene}.
However, when applying RL to the solution of deterministic optimal control problems, two major downsides arise.
First, terminal constraints cannot be explicitly accounted for, 
%MDP formulation relies on a scalar reward function, hence 
and constraint violations must be introduced in the reward function as (weighted) penalty terms. As a result,
the accuracy on constraint satisfaction is generally looser than in traditional methods for solving optimal control problems.
Second, RL is quite computationally intensive, even when applied to problems as simple as the deterministic rendezvous mission here considered. This is mainly motivated by the fact that PPO is a model-free algorithm, hence, the knowledge of the underlying (analytical) dynamical model is not exploited at all. The only way the agent can obtain satisfactory results is to acquire as much experience (i.e., samples) as possible about the environment.
In this respect, the solution of the deterministic problem here reported took about $2\div3$ hours (depending on the desired accuracy on the constraints) on a computer equipped with Intel Core i7-9700K CPU @\SI{3.60}{\giga\Hz}, while the indirect method just a few seconds.





\subsection{Robust Trajectory Design}
%commento generico


%
Besides the unperturbed, deterministic  mission scenario (labeled ${unp}$),
the following stochastic case-studies are considered:
i) state uncertainties ($st$), %$\left(f \circ g \circ h\right)^{st}$), 
ii) observation uncertainties ($obs$),
iii) control uncertainties ($ctr$),
iv) single missed thrust event ($mte,1$), and 
v) multiple missed thrust events ($mte,2$).
%
Training the \gncnet{} in one of these environments 
leads to the definition of a corresponding policy, named
%Training the \gncnet{} in each stochastic environment least to
$\pi^{unp}$, $\pi^{st}$, $\pi^{obs}$, $\pi^{ctr}$, $\pi^{mte,1}$, and $\pi^{mte,2}$, respectively.
%
%Some preliminary solutions 
%We may ``extract''
%
For each policy, the reference trajectory, which should be intended as robust to that source of uncertainty, is obtained by applying in the unperturbed environment a (deterministic) version of the policy (i.e., that always takes the action corresponding to the largest probability, instead of sampling from the probability distribution $\bm{a}\sim\pi(\cdot|\bm{s})$), and recording the commands and spacecraft states along the flight.
%the ``optimal'' reference trajectory, that is robust to that source of uncertainty, is obtained.

\begin{figure} [!htbp]
    \centering
    \includegraphics[width=0.75\textwidth, trim={0cm 0.5cm 0cm 1cm},clip]{Figures/comparison/compare2D.pdf}
    \caption{Earth-Mars trajectories corresponding to different robust policies. Differences with respect to the unperturbed policy trajectory are 
    up-scaled by  5 for illustration purposes.}
    %exaggerated by a factor 5 for illustration purposes}
    \label{fig:robust_comp} 
\end{figure}



%A robust trajectory is associated to each trained policy $\pi^i$. This %robust trajectory is computed by applying in the unperturbed environment a (deterministic) version of that policy  (i.e., that always takes the action corresponding to the largest probability, instead of sampling from the normal probability distribution $\bm{a}\sim\pi(    \bm{a}|\bm{s})$) and recording the commands and spacecraft state along the flight.
%
%
Figure~\ref{fig:robust_comp} shows the robust trajectories obtained after a training that lasts up to  $\SI{200}{\mega steps}$, that roughly corresponds to 10 $\div$ 12 computing hours.
For each case, only the best found solution during training (also accounting for the closed-loop behavior described in the next section) is reported.
To add robustness, these trajectories tend to approach Mars orbit in advance with respect to the optimal solution, so as to maximize the probability of meeting the terminal constraints even in presence of late perturbations and/or control errors.

\input{Tables/tab-robust}
%This variability in the allowed number of training stes computational budget 
%
%The numerical  solutions are now discussed
Table~\ref{tab:nom} summarizes the main features 
of these trajectories, that are, the final spacecraft mass $m_f$, constraint violations $\Delta r_f$ and 
$\Delta v_f$, and cumulative reward $J$,
%for the robust trajectories corresponding to different source of uncertainty.
as well as some environment-specific training settings.
%
The solutions corresponding to a policy trained in a stochastic environment with perturbations on either state ($\pi^{st}$), observations ($\pi^{obs}$), or control direction and magnitude ($\pi^{ctr}$) satisfy the terminal constraints within the given tolerance ($10^{-3})$. In those cases,  robustness is obtained by sacrificing less than $1 \div 2$\% of the payload mass.  
%
Instead, the solutions $\pi^{mte,1}$ and $\pi^{mte,2}$, trained in the MTE environments,
tend to slightly overcome Mars orbit, since they account, even in the unperturbed scenario, for the possible presence of MTEs, whose probability of occurrence during training has been exaggerated in this work for research purposes (at least one MTE must occur in any environment realization). Also, the final spacecraft mass obtained in these two cases is considerably worse than in the previous ones.
In all presented cases, the error on the final velocity is zero. This result should not surprise the reader. In fact, the last $\Delta V$ is computed algebraically as a difference between the final spacecraft velocity and Mars velocity. Thus, the velocity constraint is automatically satisfied whenever this (computed) $\Delta V$ has a magnitude lower than the maximum admissible by the Sims-Flanagan model (see Eq.~\ref{eq:DVmax-f}).


\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[t]{.49\textwidth}
    \centering 
       \includegraphics[width = 1\textwidth]{Figures/comparison/controls_unperturbed.pdf} %LOW - QUALITY
       \caption{Unperturbed policy.}
       \label{fig:dv_nom}
   \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{.49\textwidth}
        \centering
        \includegraphics[width = 1\textwidth]{Figures/comparison/controls_state.pdf}  %LOW - QUALITY
       \caption{State uncertainties.}
        \label{fig:dv_state}
    \end{subfigure}
     \begin{subfigure}[t]{.49\textwidth}
    \centering 
       \includegraphics[width = 1\textwidth]{Figures/comparison/controls_observation.pdf} %LOW - QUALITY
       \caption{Observation uncertainties}
       \label{fig:dv_obs}
   \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{.49\textwidth}
        \centering
        \includegraphics[width = 1\textwidth]{Figures/comparison/controls_control.pdf}  %LOW - QUALITY
       \caption{Control uncertainties.}
        \label{fig:dv_con}
    \end{subfigure}
     \begin{subfigure}[t]{.49\textwidth}
    \centering 
       \includegraphics[width = 1\textwidth]{Figures/comparison/controls_single_MTE.pdf} %LOW - QUALITY
       \caption{Single MTE.}
       \label{fig:dv_mte}
   \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{.49\textwidth}
        \centering
        \includegraphics[width = 1\textwidth]{Figures/comparison/controls_multi_MTE.pdf}  %LOW - QUALITY
       \caption{Multiple MTEs.}
        \label{fig:dv_mtes}
    \end{subfigure}
    \caption{Magnitude of the $\pmb{\Delta V}$s along the robust trajectories. Dashed lines indicate the maximum $\pmb{\Delta V}$ admitted at each time step by Sims-Flanagan model.}
    \label{fig:DVrob}
\end{figure}


Figure~\ref{fig:DVrob} shows the distribution of the magnitude of the $\Delta V$s over the flight time for the different robust trajectories. 
Dashed lines indicate the maximum allowed $\Delta V$ at each step, according to the Sims-Flanagan model (see Eq.~\eqref{eq:DVmax-k}). %allowing for a more thoughtful discussion about the respect of this constraint all along the flight.
%
As a general comment, the robust trajectories trained in the stochastic environments
show a lower $\Delta V$ magnitude at the beginning and at the end of the transfer, 
with respect to the optimal deterministic solution $\pi^{unp}$,
and, correspondingly, an higher magnitude in the central portion of the transfer.
This sub-optimal distribution of the thrust is responsible for the additional propellant consumption of the robust solutions.
%
%This difference is more evident in case of state perturbation and observation perturbations.
%
Also, the applied $\Delta V$ is consistently lower than the maximum available in all cases except the unperturbed one, where an almost bang-off-bang pattern, which is the expected solution of this kind of optimal control problems, may be recognized.
This is a distinctive feature of robust trajectories, that must satisfy the constraint on the maximum admissible value of $\Delta V$, while leaving room for efficient correction maneuvers.
As a final remark, in the two solutions obtained with policies $\pi^{mte,1}$ and $\pi^{mte,2}$ the last $\Delta V$ is considerably smaller than in the other solutions, probably because 
the two policies try to ensure the compliance with the final velocity constraint regardless of the possible presence of a MTE near the final time.




\subsection{Closed-Loop Mission Analysis}
%
%Naturally/by definition, RL provides the (putative)
%optimal closed-loop guidance policy for the environment it was trained for.
%
%This easily allow to evaluate the performance 
%
%s a final consideration, RL provides both a nominal trajectory and an ``optimal'' closed-loop guidance policy, while the indirect method does not. \hl{anche se e' possibile derivare una legge a loop chiuso al primo ordine dalle derivate di sensibilita' della soluzione - Bryson}
%%\hl{sarebbe da investigare quanto si comporta meglio/peggio di una guida a a loop-chiuso dal primo ordine dell'indiretto}
%
%\hl{the policies found by RL allows full closed-loop guidance capability.}
%
\begin{figure}[!htbp]
    \centering

    \hfill
    \begin{subfigure}[t]{.49\textwidth}
        \centering
        \includegraphics[width = 0.95\textwidth]{Figures/state/MC2D_LQ.png}  %LOW - QUALITY
       \caption{$\pi^{st}$}
        \label{fig:MC_pert}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.49\textwidth}
    \centering 
       \includegraphics[width = 0.95\textwidth]{Figures/observation/MC2D_LQ.png} %LOW - QUALITY
       \caption{$\pi^{obs}$}
       \label{fig:obs}
   \end{subfigure}%
    
    \begin{subfigure}[t]{.49\textwidth}
        \centering
        \includegraphics[width = 0.95\textwidth]{Figures/control/MC2D_LQ.png}  %LOW - QUALITY
       \caption{$\pi^{ctr}$}
        \label{fig:control}
    \end{subfigure}
    \hfill
     \begin{subfigure}[t]{.49\textwidth}
    \centering 
       \includegraphics[width = 0.95\textwidth]{Figures/MTE/MC2D_LQ.png} %LOW - QUALITY
       \caption{$\pi^{mte,1}$}
       \label{fig:MTE}
   \end{subfigure}%
    
    \begin{subfigure}[t]{.49\textwidth}
        \centering
        \includegraphics[width = 0.95\textwidth]{Figures/MTEs/MC2D_LQ.png}  %LOW - QUALITY
       \caption{$\pi^{mte,2}$}
        \label{fig:MTEs}
    \end{subfigure}
    \hfill
        \begin{subfigure}[t]{.49\textwidth}
    \centering 
       \includegraphics[width = 0.95\textwidth]{Figures/nominal/MC2D_state_LQ.png} %LOW - QUALITY
       \caption{$\pi^{unp}$}
       \label{fig:MC_det}
   \end{subfigure}%
    \caption{Monte Carlo simulations realized by running each policy in the correspondingly-perturbed environment, except for the unperturbed policy, which is run in the state-perturbed one. Differences are exaggerated by a factor 5 for illustration purposes.}
    \label{fig:MCs}
\end{figure}

The closed-loop performance of the \gncnet{s} in their respective (stochastic) training environment are measured by using a Monte Carlo approach that consists in running each state-feedback policy in 500 randomly-generated environment realizations, or episodes. 
%
%
Figure~\ref{fig:MCs} shows the results of the Monte Carlo campaigns in terms of spacecraft trajectory in each randomly-generated episode. Specifically, in each figure, the dark-blue line represents the robust trajectory, with the light-blue arrows indicating the $\Delta V$s, while each gray line represents the trajectory obtained in one of the randomly-generated episodes. % (the differences with respect to the robust trajectory are exaggerated 5 times for illustration purposes). 
One may notice that, for policies $\pi^{st}$, $\pi^{obs}$, $\pi^{ctr}$ and $\pi^{mte,1}$, the Monte Carlo generated trajectories have a greater dispersion in the central part of the mission, which tends to reduce, and disappear almost entirely, while approaching the final time, because of the imposed terminal constraints. This is not completely true for the case of multiple MTEs, where a small number of trajectories (15 out of 500) clearly miss the target by far.

\input{Tables/tab-MC}
Table~\ref{tab:MC} shows that RL is able to cope with all these different stochastic scenarios 
effectively. %with an high success rate. 
Indeed, despite the severity of the considered perturbations/uncertainties, the success rate (that is, the percentage of solutions that meet final constraints within the prescribed accuracy) is rather high, over 70\% in most cases and up to 80\% when only additive Gaussian state perturbations are considered.
%
%\hl{non so cosa dire sulla massa}
%
%\input{Tables/tab-unpMC}
For the sake of comparison, we also reported the results obtained by running policy $\pi^{unp}$ in the state-perturbed stochastic environment (Fig.~\ref{fig:MC_det}).
While the differences between the robust trajectories corresponding to policy $\pi^{unp}$ and $\pi^{st}$ seem minimal, the effects in the closed-loop simulations are apparent.
Indeed, in none of the episodes the policy $\pi^{unp}$ was able to reach the imposed accuracy on terminal state, while policy $\pi^{st}$ succeeds in the $80\%$ of the cases.
%
Similar results are obtained when running the policy $\pi^{unp}$ in any of the proposed perturbed (stochastic) environments.
More precisely, the success rate is zero for both the state- and observation-uncertainty environments, while in case of control uncertainties on thrust magnitude/direction is 8\%, and almost double in case of single (18.8\%) or multiple (16.8\%) MTEs.

The preliminary results found with policies $\pi^{mte,1}$ and $\pi^{mte,2}$ 
stressed that RL performance deteriorates substantially in the presence of MTEs.
By looking at Figure~\ref{fig:errors}, it is clear that, in most cases ($69.8\%$ with a single MTE, $70.4\%$ with multiple MTEs) the policy manages to recover from the complete absence of thrust, and meets the final constraints within the imposed tolerance ($10^{-3}$). However, in a few unfortunate scenarios, the MTE occurs in ``crucial points'' of the trajectory, that is, near final time, and the policy is not able to compensate for the missing $\Delta V$s in any way. As a result, the terminal constraints cannot be met. This fact is confirmed by the high variance obtained on the constraint violation in both mission scenarios (single and multiple MTEs). Analogously, the drop in payload mass (Fig.~\ref{fig:mass}) highlights what are the most critical points in terms of thrust efficiency. The looser satisfaction of the terminal constraints is deemed responsible for the final rise in the achieved payload mass and might be misleading.


\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[t]{.47\textwidth} %45
    \centering 
       \includegraphics[width = 1\textwidth]{Figures/MTE/MTE_error.pdf} %LOW - QUALITY
       \caption{Terminal constraint violation.}
       \label{fig:errors}
   \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{.51\textwidth} %54
        \centering
        \includegraphics[width = 1\textwidth]{Figures/MTE/MTE_mass.pdf}  %LOW - QUALITY
       \caption{Final spacecraft mass.}
        \label{fig:mass}
    \end{subfigure}
    \caption{Terminal constraint violation (a) and final spacecraft mass (b) obtained with policy $\pmb{\pi^{mte,1}}$ by varying the MTE location $\pmb{\hat{k}}$.}
    \label{fig:mte_analysis}
\end{figure}



















 












%state: min = 552.44, max = 617.12obs: min = 550.11, max = 605.87ctr: min = 588.46, max = 592.90mte 1: min = 573.58, max = 590.32mte 2: min = 537.71, max = 578.92
  

==> Tables/tab-1.tex <==
\begin{table}[htbp]
	%\fontsize{10}{10}\selectfont
    \caption{Problem data.}
   \label{tab:data}
        \centering 
   \begin{tabular}{c c} % Column formatting, 
      \hline 
      Variable  & Value\\
      \hline 
      $N$       & 40 \\
      $t_f,\, \si{days}$     &  $358.79$ \\
      $T_{max},\, \si{\kilo\newton}$ &  $0.50$ \\
      $u_{eq},\, \si{\kilo\meter/\second}$  &  $19.6133$ \\
      $m_0,\, \si{\kilo\gram}$ & $1000$ \\
      $\mu_\Sun,\,  \si{\kilo\meter^3/\second^2}$ & $132712440018$ \\
      $\bm{r}_\Earth,\, \si{\kilo\meter}$ & $[-140699693,\, -51614428,\, 980]^T$\\
      $\bm{v}_\Earth,\, \si{\kilo\meter/\second}$ & $[9.774596,\, -28.07828,\, 4.337725 \times 10^{-4}]^T$\\
      $\bm{r}_\Mars,\, \si{\kilo\meter}$ & $[-172682023,\, 176959469,\, 7948912]^T$\\
      $\bm{v}_\Mars,\,\si{\kilo\meter/\second}$ & $[-16.427384,\, -14.860506,\, 9.21486 \times 10^{-2}]^T$\\
      \hline
   \end{tabular}
\end{table}



==> Tables/tab-unpMC.tex <==
\begin{table}[!htbp]
	%\fontsize{10}{10}\selectfont
    \caption{Performance of policy $\pi^{unp}$ in terms of satisfaction ratio, that is number of cases where the terminal constraints on final position and velocity are respected out of 500 runs, when deployed in %applied to
    various perturbed (stochastic) environments.
    }
   \label{tab:unpMC}
        \centering 
    {\renewcommand{\arraystretch}{1.2}
   \begin{tabular}{l  r r } % Column formatting, 
   \hline 
   \multirow{2}{*}{Perturbation} & \multicolumn{2}{c}{Success rate [\%]} \\
    & Position constraint & Velocity constraint \\
     %Perturbation & $\Delta r_f/r_\Mars$  SR [\%] & $\Delta v_f/v_\Mars$  SR [\%] \\
    % & SR [\%] & SR [\%] \\
      \hline 
      state & $0.0$  & $50.2$  \\
      observations & $0.0$ & $45.8$\\
      control &  $12.8$ & $64.4$\\
      single MTE & $18.8$ & $35.0$\\
      multiple MTEs & $16.8$ & $33.8$\\
      \hline 
   \end{tabular}
   }
\end{table}

%        r     v
%state : 0   50.2
%observation: 0 45.8
%control: 12.8 64.4
%MTE:  18.8 35.0
%MTEs: 16.8 33.8
